Neural Fingerprints for Malware Analysis: An Image-Based Metric Learning Approach with Application to Cross-Domain Classification

Identifying the family of a newly observed malware sample is a core task in threat intelligence, yet conventional classifiers must be retrained whenever a new family appears. This chapter develops an image-based metric learning approach that instead learns to extract discriminative neural fingerprints--fixed-length embeddings--from malware-as-image representations, so that family membership can be determined by nearest-neighbor search in the embedding space. The central advantage of this formulation is zero-shot capability: because the learned embedding induces a similarity metric rather than a fixed set of class boundaries, families that were never seen during training can be recognized by comparison against a gallery, with no retraining. We demonstrate this directly by training an encoder on MalNet-Images-Tiny and MalImg combined (453 families, 96,769 images) and evaluate it zero-shot on a held-out 17-family grayscale dataset with no family overlap. Using a lightweight CNN with multi-proxy anchor loss, this model attains 73.1% retrieval@1 and 90.5% open-set AUROC on families the encoder has never seen. We benchmark our embedding approach against two conventional paradigms in a same-domain setting, where all three are competitive at classifying malware into families. We further show that the learned embeddings transfer across datasets. Unlike classifiers, our embedding approach also yields interpretable similarity scores and scales to large galleries via Facebook AI Similarity Search (FAISS). Finally, we provide a comprehensive evaluation of the learned embedding space using retrieval@k, cluster purity, silhouette score, separation ratio, few-shot accuracy, and open-set detection metrics, along with robustness analysis under image perturbations.

==> figures/bar_accuracy.tex <==
\begin{tikzpicture}[scale=0.8, every node/.style={scale=1.0}]
\pgfkeys{/pgf/number format/.cd,1000 sep={}}
\begin{axis}[%axis x line*=bottom,
	%bar shift=0pt,
	axis y line*=left,
        width  = 0.55*\textwidth,
        height = 8.0cm,
        ymin=0.58,ymax=1.035,
%        ytick={0.0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
        ytick={0.60, 0.70, 0.80, 0.90, 1.00},
        major x tick style = transparent,
        ybar=5*\pgflinewidth,
%        bar width=15.0pt,
        bar width=22.0pt,
        bar shift=-12.75pt,
%        ymajorgrids = true,
%        xlabel = {Learning technique},
        ylabel = {Test accuracy},
        ylabel style = {scale = 0.95},
%        symbolic x coords={MLR, SVC, MLP, CNN, RNN, LSTM, RF, XGBoost},
%        xticklabels={MLR, SVC, MLP, CNN, RNN, LSTM, RF, XGBoost},
        symbolic x coords={A, B, C},
        xticklabels={Classic ML (SVM), DL (ResNet-18), Metric learning},
	y tick label style={scale=0.95,
%		rotate=60,
    		/pgf/number format/.cd,
   		fixed,
   		fixed zerofill,
%		sep=,
    		precision=2},
%	yticklabel pos=right,
        xtick = data,
        x tick label style={scale=1.0,        	
        		rotate=60,
%		font=\small,
		anchor=north east,
		inner sep=0mm
		},
%		font=\small},
%        scaled y ticks = false,
	%%%%% numbers on bars and rotated
        nodes near coords,
        every node near coord/.append style={rotate=90, scale=0.875,
        								   anchor=west, 
								   %font=\footnotesize,
								   /pgf/number format/.cd,
								   fixed,
								   fixed zerofill,
%								   sep=,
								   precision=3},
        %%%%%
%        enlarge x limits=0.03,
%        enlarge x limits=0.06,
        enlarge x limits=0.265,
        legend cell align=left,
        legend pos=south east,
%        legend style={
%%                at={(1,1.05)},
%%                anchor=south east,
%%	        nodes={rotate=90},%%%%% rotate text in legend
%%                at={(0.125,0)},
%%                at={(0.125,0)},
%%                at={(0.8775,0)},
%                at={(0.82,0.56)},
%                anchor=south,
%                column sep=1ex
%        },
]
\addplot [fill=blue,opacity=1.00]
coordinates {
(A, 0.860)
(B, 0.910)
(C, 0.940)
}; \label{AAA}
\end{axis}
\begin{axis}[%axis x line*=bottom,
	%bar shift=0pt,
	axis y line*=right,
        width  = 0.55*\textwidth,
        height = 8.0cm,
        ymin=0.0,ymax=2.65,
%        ytick={0.0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
        ytick={0.0, 0.5, 1.0, 1.5, 2.0, 2.5},
        major x tick style = transparent,
        ybar=5*\pgflinewidth,
%        bar width=15.0pt,
        bar width=22.0pt,
        bar shift=12.75pt,
%        ymajorgrids = true,
%        xlabel = {Learning technique},
        ylabel = {Training time (hours)},
        ylabel style = {scale = 0.95},
%        symbolic x coords={MLR, SVC, MLP, CNN, RNN, LSTM, RF, XGBoost},
%        xticklabels={MLR, SVC, MLP, CNN, RNN, LSTM, RF, XGBoost},
        symbolic x coords={A, B, C},
%        xticklabels={Classic ML (SVM), DL (ResNet-18), Metric learning},
	xticklabels=empty,
	y tick label style={scale=0.95,
%		rotate=60,
    		/pgf/number format/.cd,
   		fixed,
   		fixed zerofill,
%		sep=,
    		precision=2},
%	yticklabel pos=right,
%        xtick = data,
%        x tick label style={scale=1.0,        	
%        		rotate=60,
%%		font=\small,
%		anchor=north east,
%		inner sep=0mm
%		},
%		font=\small},
%        scaled y ticks = false,
	%%%%% numbers on bars and rotated
        nodes near coords,
        every node near coord/.append style={rotate=90, scale=0.875,
        								   anchor=west, 
								   %font=\footnotesize,
								   /pgf/number format/.cd,
								   fixed,
								   fixed zerofill,
%								   sep=,
								   precision=1},
        %%%%%
%        enlarge x limits=0.03,
%        enlarge x limits=0.06,
        enlarge x limits=0.265,
        legend cell align=left,
        legend pos=south east,
%        legend style={
%%                at={(1,1.05)},
%%                anchor=south east,
%%	        nodes={rotate=90},%%%%% rotate text in legend
%%                at={(0.125,0)},
%%                at={(0.125,0)},
%%                at={(0.8775,0)},
%                at={(0.82,0.56)},
%                anchor=south,
%                column sep=1ex
%        },
]
\addlegendimage{/pgfplots/refstyle=AAA}
\addlegendentry{Accuracy}
\addplot [fill=red,opacity=1.00]
coordinates {
(A, 0.1)
(B, 2.3)
(C, 2.3)
};
\addlegendentry{Time}
\end{axis}
\end{tikzpicture}


==> figures/bar_time.tex <==
\begin{tikzpicture}[scale=0.8, every node/.style={scale=1.0}]
\pgfkeys{/pgf/number format/.cd,1000 sep={}}
\begin{axis}[%axis x line*=bottom,
	%bar shift=0pt,
        width  = 0.55*\textwidth,
        height = 8.0cm,
        ymin=0.0,ymax=2.65,
%        ytick={0.0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
        ytick={0.0, 0.5, 1.0, 1.5, 2.0, 2.5},
        major x tick style = transparent,
        ybar=5*\pgflinewidth,
%        bar width=15.0pt,
        bar width=32.0pt,
%        ymajorgrids = true,
%        xlabel = {Learning technique},
        ylabel = {Training time (hours)},
        ylabel style = {scale = 0.95},
%        symbolic x coords={MLR, SVC, MLP, CNN, RNN, LSTM, RF, XGBoost},
%        xticklabels={MLR, SVC, MLP, CNN, RNN, LSTM, RF, XGBoost},
        symbolic x coords={A, B, C},
        xticklabels={Classic ML (SVM), DL (ResNet-18), Metric learning},
	y tick label style={scale=0.95,
%		rotate=60,
    		/pgf/number format/.cd,
   		fixed,
   		fixed zerofill,
%		sep=,
    		precision=2},
%	yticklabel pos=right,
        xtick = data,
        x tick label style={scale=1.0,        	
        		rotate=60,
%		font=\small,
		anchor=north east,
		inner sep=0mm
		},
%		font=\small},
%        scaled y ticks = false,
	%%%%% numbers on bars and rotated
        nodes near coords,
        every node near coord/.append style={rotate=90, scale=0.875,
        								   anchor=west, 
								   %font=\footnotesize,
								   /pgf/number format/.cd,
								   fixed,
								   fixed zerofill,
%								   sep=,
								   precision=1},
        %%%%%
%        enlarge x limits=0.03,
%        enlarge x limits=0.06,
        enlarge x limits=0.20,
        legend cell align=left,
        legend pos=south east,
%        legend style={
%%                at={(1,1.05)},
%%                anchor=south east,
%%	        nodes={rotate=90},%%%%% rotate text in legend
%%                at={(0.125,0)},
%%                at={(0.125,0)},
%%                at={(0.8775,0)},
%                at={(0.82,0.56)},
%                anchor=south,
%                column sep=1ex
%        },
]
\addplot [fill=red,opacity=1.00]
coordinates {
(A, 0.1)
(B, 2.3)
(C, 2.3)
};
\end{axis}
\end{tikzpicture}

